Keypoint-Augmented Self-Supervised Learning for Medical Image Segmentation with Limited Annotation

Pretraining CNN models (i.e., UNet) through self-supervision has become a powerful approach to facilitate medical image segmentation under low annotation regimes. Recent contrastive learning methods encourage similar global representations when the same image undergoes different transformations, or enforce invariance across different image/patch features that are intrinsically correlated. However, CNN-extracted global and local features are limited in capturing long-range spatial dependencies that are essential in biological anatomy. To this end, we present a keypoint-augmented fusion layer that extracts representations preserving both short- and long-range self-attention. In particular, we augment the CNN feature map at multiple scales by incorporating an additional input that learns long-range spatial self-attention among localized keypoint features. Further, we introduce both global and local self-supervised pretraining for the framework. At the global scale, we obtain global representations from both the bottleneck of the UNet, and by aggregating multiscale keypoint features. These global features are subsequently regularized through image-level contrastive objectives. At the local scale, we define a distance-based criterion to first establish correspondences among keypoints and encourage similarity between their features. Through extensive experiments on both MRI and CT segmentation tasks, we demonstrate the architectural advantages of our proposed method in comparison to both CNN and Transformer-based UNets, when all architectures are trained with randomly initialized weights. With our proposed pretraining strategy, our method further outperforms existing SSL methods by producing more robust self-attention and achieving state-of-the-art segmentation results. The code is available at https://github.com/zshyang/kaf.git.

==> app_figures/connections.tex <==
\begin{figure*}[h]
\includegraphics[width=\linewidth]{app_assest/connections.png}
\centering
\caption{ 
\textbf{The closest and furthest keypoints from the query keypoints, are computed using our method.} The visualization indicates that, in the network's deeper layers, keypoints tend to form connections with points sharing similar labels, illustrating the semantic learning capabilities of our approach. 
}
\label{app-fig:connections}
\end{figure*}

==> app_figures/sparse.tex <==
\begin{figure*}[h]
\includegraphics[width=\linewidth]{app_assest/sparse.png}
\centering
\caption{ 
Visualization of the similarity map on both the convolution feature map from blocks 1, 2, 3, 4 and the keypoint dense convolution features. 
The importance of the fourth layer is highlighted by its dense convolution features, where the ratio between the background and the featured positions is larger than other layers, illustrating its significant role in the network's performance
}
\label{app-fig:sparse}
\end{figure*}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> rebuttal_figures/corr.tex <==
\begin{figure*} [t]
    \includegraphics[width=0.9\linewidth]{rebuttal_assest/corr.png}
    \centering
    \caption{
       Sensitivity analysis of the Manhattan distance, illustrating the correspondence found under the specified Manhattan distance threshold."
    }
    \label{fig:corr}
\end{figure*}

==> rebuttal_figures/seg.tex <==
\begin{figure*} [tp]
    \centering
    \includegraphics[width=1.0\linewidth]{rebuttal_assest/seg.png}
    \caption{
       \textbf{Revised Figure 1.}
    }
    \label{fig:seg}
\end{figure*}
